On the efficiency of polar-like decoding for symmetric codes

The recently introduced polar codes constitute a breakthrough in coding theory due to their capacityachieving property. This goes hand in hand with a quasilinear construction, encoding, and successive cancellation list decoding procedures based on the Plotkin construction. The decoding algorithm can be applied with slight modifications to Reed-Muller or eBCH codes, that both achieve the capacity of erasure channels, although the list size needed for good performance grows too fast to make the decoding practical even for moderate block lengths. The key ingredient for proving the capacity-achieving property of Reed-Muller and eBCH codes is their group of symmetries. It can be plugged into the concept of Plotkin decomposition to design various permutation decoding algorithms. Although such techniques allow to outperform the straightforward polar-like decoding, the complexity stays impractical. In this paper, we show that although invariance under a large automorphism group is valuable in a theoretical sense, it also ensures that the list size needed for good performance grows exponentially. We further establish the bounds that arise if we sacrifice some of the symmetries. Although the theoretical analysis of the list decoding algorithm remains an open problem, our result provides an insight into the factors that impact the decoding complexity.

==> fact0raw.tex <==
	\tikzstyle{tnode}  = [radius=0.05, red, thick, fill=red];
		\tikzstyle{lineP}  = [-, thick,  black];
		\coordinate  (0) at (    0,    0);
		\coordinate  (1) at (	0,		-0.75);
		\coordinate  (2) at (	0,		-1.5);
		\coordinate  (3) at (	0,		-2.25);
		\coordinate  (4) at (	0,		-3);
		\coordinate  (5) at (	0,		-3.75);
		\coordinate  (6) at (	0,		-4.5);
		\coordinate  (7) at (	0,		-5.25);
		
		\coordinate  (8) at (    1.5,     0);
		\coordinate  (9) at (	1.5,	 -0.75);
		\coordinate  (10) at (	1.5,	 -1.5);
		\coordinate  (11) at (	1.5,	 -2.25);
		\coordinate  (12) at (	1.5,	 -3);
		\coordinate  (13) at (	1.5,	 -3.75);
		\coordinate  (14) at (	1.5,	 -4.5);
		\coordinate  (15) at (	1.5,	 -5.25);
		
		\coordinate  (16) at (    3.,    0);
		\coordinate  (17) at (	3.,		-0.75);
		\coordinate  (18) at (	3.,		-1.5);
		\coordinate  (19) at (	3.,		-2.25);
		\coordinate  (20) at (	3.,		-3);
		\coordinate  (21) at (	3.,		-3.75);
		\coordinate  (22) at (	3.,		-4.5);
		\coordinate  (23) at (	3.,		-5.25);	
		
		\coordinate  (24) at (    4.5,    0);
		\coordinate  (25) at (	4.5,	 -0.75);
		\coordinate  (26) at (	4.5,	 -1.5);
		\coordinate  (27) at (	4.5,	 -2.25);
		\coordinate  (28) at (	4.5,	 -3);
		\coordinate  (29) at (	4.5,	 -3.75);
		\coordinate  (30) at (	4.5,	 -4.5);
		\coordinate  (31) at (	4.5,	 -5.25);
		
		\draw  (0)  [tnode] circle;
		\draw  (1) [tnode] circle;
		\draw  (2) [tnode] circle;
		\draw  (3) [tnode] circle;
		\draw  (4) [tnode] circle;
		\draw  (5) [tnode] circle;
		\draw  (6) [tnode] circle;
		\draw  (7) [tnode] circle;
		\draw  (8) [tnode] circle;
		\draw  (9) [tnode] circle;
		\draw (10) [tnode] circle;
		\draw (11) [tnode] circle;
		\draw (12) [tnode] circle;
		\draw (13) [tnode] circle;
		\draw (14) [tnode] circle;
		\draw (15) [tnode] circle;
		\draw (16) [tnode] circle;
		\draw (17) [tnode] circle;
		\draw (18) [tnode] circle;
		\draw (19) [tnode] circle;
		\draw (20) [tnode] circle;
		\draw (21) [tnode] circle;
		\draw (22) [tnode] circle;
		\draw (23) [tnode] circle;
		\draw (24) [tnode] circle;
		\draw (25) [tnode] circle;
		\draw (26) [tnode] circle;
		\draw (27) [tnode] circle;
		\draw (28) [tnode] circle;
		\draw (29) [tnode] circle;
		\draw (30) [tnode] circle;
		\draw (31) [tnode] circle;		
		
		\draw [lineP] (0) -- (24);
		\draw [lineP] (1) -- (25);
		\draw [lineP] (2) -- (26);
		\draw [lineP] (3) -- (27);
		\draw [lineP] (4) -- (28);
		\draw [lineP] (5) -- (29);
		\draw [lineP] (6) -- (30);
		\draw [lineP] (7) -- (31);
		
		
		\draw [lineP] (1) -- (8);
		\draw [lineP] (3) -- (10);
		\draw [lineP] (5) -- (12);
		\draw [lineP] (7) -- (14);
		
		\draw [lineP] (10) -- (16);
		\draw [lineP] (11) -- (17);
		\draw [lineP] (14) -- (20);
		\draw [lineP] (15) -- (21);
		
		\draw [lineP] (20) -- (24);
		\draw [lineP] (21) -- (25);
		\draw [lineP] (22) -- (26);
		\draw [lineP] (23) -- (27);

==> fact1raw.tex <==
\tikzstyle{tnode}  = [radius=0.05, red, thick, fill=red];
		\tikzstyle{lineP}  = [-, thick,  black];
		\coordinate  (24)   at (    0,    0);
		\coordinate  (25)   at (	0,		-0.75);
		\coordinate  (26)   at (	0,		-1.5);
		\coordinate  (27)   at (	0,		-2.25);
		\coordinate  (28)   at (	0,		-3);
		\coordinate  (29)   at (	0,		-3.75);
		\coordinate  (30)   at (	0,		-4.5);
		\coordinate  (31)   at (	0,		-5.25);
		
		\coordinate  (0) at (    1.5,     0);
		\coordinate  (1) at (	1.5,	 -0.75);
		\coordinate  (2) at (	1.5,	 -1.5);
		\coordinate  (3) at (	1.5,	 -2.25);
		\coordinate  (4) at (	1.5,	 -3);
		\coordinate  (5) at (	1.5,	 -3.75);
		\coordinate  (6) at (	1.5,	 -4.5);
		\coordinate  (7) at (	1.5,	 -5.25);
		
		\coordinate (8)  at (    3.,    0);
		\coordinate (9)  at (	3.,		-0.75);
		\coordinate (10) at (	3.,		-1.5);
		\coordinate (11) at (	3.,		-2.25);
		\coordinate (12) at (	3.,		-3);
		\coordinate (13) at (	3.,		-3.75);
		\coordinate (14) at (	3.,		-4.5);
		\coordinate (15) at (	3.,		-5.25);	
		
		\coordinate (16) at (    4.5,    0);
		\coordinate (17) at (	4.5,	 -0.75);
		\coordinate (18) at (	4.5,	 -1.5);
		\coordinate (19) at (	4.5,	 -2.25);
		\coordinate (20) at (	4.5,	 -3);
		\coordinate (21) at (	4.5,	 -3.75);
		\coordinate (22) at (	4.5,	 -4.5);
		\coordinate (23) at (	4.5,	 -5.25);
		
		\draw  (0)  [tnode] circle;
		\draw  (1) [tnode] circle;
		\draw  (2) [tnode] circle;
		\draw  (3) [tnode] circle;
		\draw  (4) [tnode] circle;
		\draw  (5) [tnode] circle;
		\draw  (6) [tnode] circle;
		\draw  (7) [tnode] circle;
		\draw  (8) [tnode] circle;
		\draw  (9) [tnode] circle;
		\draw (10) [tnode] circle;
		\draw (11) [tnode] circle;
		\draw (12) [tnode] circle;
		\draw (13) [tnode] circle;
		\draw (14) [tnode] circle;
		\draw (15) [tnode] circle;
		\draw (16) [tnode] circle;
		\draw (17) [tnode] circle;
		\draw (18) [tnode] circle;
		\draw (19) [tnode] circle;
		\draw (20) [tnode] circle;
		\draw (21) [tnode] circle;
		\draw (22) [tnode] circle;
		\draw (23) [tnode] circle;
		\draw (24) [tnode] circle;
		\draw (25) [tnode] circle;
		\draw (26) [tnode] circle;
		\draw (27) [tnode] circle;
		\draw (28) [tnode] circle;
		\draw (29) [tnode] circle;
		\draw (30) [tnode] circle;
		\draw (31) [tnode] circle;
		\draw [lineP] (0) -- (8);
		\draw [lineP] (1) -- (8);
		\draw [lineP] (1) -- (9);
		\draw [lineP] (2) -- (10);
		\draw [lineP] (3) -- (10);
		\draw [lineP] (3) -- (11);
		\draw [lineP] (4) -- (12);
		\draw [lineP] (5) -- (12);
		\draw [lineP] (5) -- (13);
		\draw [lineP] (6) -- (14);
		\draw [lineP] (7) -- (14);
		\draw [lineP] (7) -- (15);
		
		\draw [lineP] (8) -- (16);
		\draw [lineP] (10) -- (16);
		\draw [lineP] (10) -- (18);
		\draw [lineP] (9) -- (17);
		\draw [lineP] (11) -- (17);
		\draw [lineP] (11) -- (19);
		\draw [lineP] (12) -- (20);
		\draw [lineP] (14) -- (20);
		\draw [lineP] (14) -- (22);
		\draw [lineP] (13) -- (21);
		\draw [lineP] (15) -- (21);
		\draw [lineP] (15) -- (23);
		
		\draw [lineP] (16) -- (24);
		\draw [lineP] (20) -- (28);
		\draw [lineP] (17) -- (25);
		\draw [lineP] (21) -- (29);
		\draw [lineP] (18) -- (26);
		\draw [lineP] (22) -- (30);
		\draw [lineP] (19) -- (27);
		\draw [lineP] (23) -- (31);
		\draw [lineP] (28) -- (0);
		\draw [lineP] (29) -- (1);
		\draw [lineP] (30) -- (2);
		\draw [lineP] (31) -- (3);

==> factgraph0.tex <==
\begin{tikzpicture}[thick,scale=0.55, every node/.style={scale=0.6}]
		\input{fact0raw.tex}
		
		\draw node at (    5,    0) {{\color{black}$u_0$}};
		\draw node at (	5,		-0.75)  {{\color{black}$u_1$}};
		\draw node at (	5,		-1.5)  {{\color{black}$u_2$}};
		\draw node at (	5,		-2.25)  {{\color{black}$u_3$}};
		\draw node at (	5,		-3)  {{\color{black}$u_4$}};
		\draw node at (	5,		-3.75)  {{\color{black}$u_5$}};
		\draw node at (	5,		-4.5)  {{\color{black}$u_6$}};
		\draw node at (	5,		-5.25)  {{\color{black}$u_7$}};
		
		\draw node at (    -0.5,    0) {{\color{black}$y_0$}};
		\draw node at (	-0.5,		-0.75)  {{\color{black}$y_1$}};
		\draw node at (	-0.5,		-1.5)  {{\color{black}$y_2$}};
		\draw node at (	-0.5,		-2.25)  {{\color{black}$y_3$}};
		\draw node at (	-0.5,		-3)  {{\color{black}$y_4$}};
		\draw node at (	-0.5,		-3.75)  {{\color{black}$y_5$}};
		\draw node at (	-0.5,		-4.5)  {{\color{black}$y_6$}};
		\draw node at (	-0.5,		-5.25)  {{\color{black}$y_7$}};
\end{tikzpicture}

==> factgraph1.tex <==
\begin{tikzpicture}[thick,scale=0.55, every node/.style={scale=0.6}]
		\input{fact1raw.tex}		
		
		\draw node at (    5,    0) {{\color{black}$u_0$}};
		\draw node at (	5,		-0.75)  {{\color{black}$u_1$}};
		\draw node at (	5,		-1.5)  {{\color{black}$u_2$}};
		\draw node at (	5,		-2.25)  {{\color{black}$u_3$}};
		\draw node at (	5,		-3)  {{\color{black}$u_4$}};
		\draw node at (	5,		-3.75)  {{\color{black}$u_5$}};
		\draw node at (	5,		-4.5)  {{\color{black}$u_6$}};
		\draw node at (	5,		-5.25)  {{\color{black}$u_7$}};
		
		\draw node at (    -0.5,    0) {{\color{black}$y_0$}};
		\draw node at (	-0.5,		-0.75)  {{\color{black}$y_1$}};
		\draw node at (	-0.5,		-1.5)  {{\color{black}$y_2$}};
		\draw node at (	-0.5,		-2.25)  {{\color{black}$y_3$}};
		\draw node at (	-0.5,		-3)  {{\color{black}$y_4$}};
		\draw node at (	-0.5,		-3.75)  {{\color{black}$y_5$}};
		\draw node at (	-0.5,		-4.5)  {{\color{black}$y_6$}};
		\draw node at (	-0.5,		-5.25)  {{\color{black}$y_7$}};
\end{tikzpicture}

==> polarconstr.tex <==
%\subsection{Derivative-constrained polar codes}
%In section \ref{ss:affsym} it is observed that the best projection $\mathcal C^{(e^*)}$ for polar codes constructed for Gaussian channel has rate much smaller than the capacity of the underlying channel. This along with the fact that the practical SNR region for polar codes corresponds to much higher capacity than the code rate suggests that we would still get good list decoding performance if we artificially increase this dimension. Let $\mathcal F_k$ be a set of frozen symbols for polar code of dimension $k$. The dimension $\tilde k^*$ of $\mathcal C^{(e^*)}$ is the number of indices $0\le i < n/2$ that are not in $\mathcal F_k$. A \textit{derivative-constrained} polar code of dimension $k$ with constraint parameter $s$ is constructed by choosing the set $\mathcal F$ to contains the indices of worst bit subchannels while satisfying the constraint $\dim \mathcal C^{(e^*)}=\tilde k^*+s$, i.e., $s$ indices $j'_i< n/2$ are replaced with $s$ indices $j''_i\ge n/2$, where $j'_i$ and $j''_i$ correspond to the best and the worst bit subchannels, respectively.
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth]{plots/FER_10_512_b.eps}
%	\caption{Derivative-constrained $(1024,512)$ polar codes}
%	\label{fig:dcpolar}
%\end{figure}

%Figure \ref{fig:dcpolar} demonstrates the performance of derivative-constrained codes, where Gaussian approximation at $E_b/N_0=2dB$ is used to estimate the subchannel reliabilities and list size $L=32$ is used for decoding. The proposed approach allows to construct better codes and by tweaking $s$ there is a trade-off between the performance in high- and low-SNR region. 

%\subsection{Projection-aggegation decoding in BEC}
%In case of highly symmetrical codes, one might consider the application of projection-aggregation (PA) algorithm \cite{ye2019recursive}. For demonstration purposes, we use its variation for erasure channel, where bit-MAP decoder is available. Given the received vector $y$, PA operates as follows:
%\begin{enumerate}
%	\item For each nonzero $b$, compute $y^{(b)},y^{(b)}_i=y_i\oplus y_{i+b}$. $y^{(b)}_i$ is an erasure if either of $y_i,y_{i+b}$ is.
%	\item Perform bit-MAP decoding to recover $c^{(b)}$
%	\item If $c^{(b)}_i$ is recovered and only one element of pair $y_i,y_{i+b}$ is erased, we recover another one 
%	\item If all bits of $c$ are recovered, return $c$
%	\item If no new bits of $c$ are recovered from previous iteration, randomly resolve one of the erased bits
%	\item Go to step 1.
%\end{enumerate}

==> struct.tex <==
\section{Structure of partially symmetric codes}
Let us define $\check{\mathcal C}_{m,t}$ as the code obtained using the procedure from Section \ref{ssDesign}.

\begin{prop}
	For any $\check{\mathcal C}_{m,t}$ holds $\mathcal T_m\in \aut(\check{\mathcal C}_{m,t})$.
\end{prop}
This property follows directly from the code construction. Consider a monomial $x^v\in M_{\check{\mathcal C}_{m,t}}$ and assume it has $\tilde l$ variables in $\mathcal M_t$. Any divisor of $x^v$ has $\le \tilde l$ variables in $\mathcal M_t$ and smaller degree, so it cannot be removed from $M_{\check{\mathcal C}_{m,t}}$ nefore $x^v$ in the construction process. As a consequence \cite{bardet2016algebraic}, the dual code $\check{\mathcal C}_{m,t}^\bot$ is also monomial and $\mathcal T_m\in \aut(\check{\mathcal C}_{m,t}^\bot)$.

\begin{prop}
	$\check{\mathcal C}_{m,t}$ is invariant w.r.t. any permutation on sets $\{x_1,\dots,x_{t}\}$ and $\{x_{t+1},\dots,x_{m}\}$.
\end{prop}
It is sufficient to observe that for any $d,l$ all degree-$d$ monomials with $l$ variables in $\mathcal M_t$ (and $d-l$ variables in $\mathcal M_t^c$) are either in $M_{\check{\mathcal C}_{m,t}}$ or its complement.


Note that in some cases codes $\check{\mathcal C}_{m,t}$ might coincide with the ones from \cite{kamenev2019polar} (which are for some choice of parameters invariant w.r.t. $\{x_0,\dots,x_{t}\}$, but are optimized for SC decoding error probability rather than the projected code dimensions), but contrary to them the construction of $\check{\mathcal C}_{m,t}$ is channel-independent.

\begin{prop}
	For any $e_i\in \mathcal H_t$ code $\check{\mathcal C}_{m,t}^{(e_i)}$ achieves $\tilde k^*_{m-1,t-1}$.
\end{prop}
Consider the generating set of code $\check{\mathcal C}_{m,t}$. It contains all monomials of two types:
\begin{enumerate}
	\item With less than $\hat l$ variables in $\mathcal M_t$;
	\item With exactly $\hat l$ variables in $\mathcal M_t$ and total degree less than $\hat d$
\end{enumerate}
for some $\hat l, \hat d$. When we take the derivative in the direction $e_i\in \mathcal H_t$, the monomials of first type now have less than $\hat l-1$ variables in $\mathcal M_t\setminus \{x_i\}$ and the monomials of second type now have exactly $\hat l-1$ variables in $\mathcal M_t\setminus \{x_i\}$ and total degree less than $\hat d-1$. The only thing left here is to notice that this matches exactly the description of code $\check{\mathcal C}_{m-1,t-1}$.

%\begin{conj}
%	Consider a code $\tilde{\mathcal C}_{m,t}$ obtained using the method from section \ref{ssFin}. For any $e_i,e_j\in \mathcal H_t$ codes $\tilde{\mathcal C}_{m,t}^{(e_i)}$ and $\tilde{\mathcal C}_{m,t}^{(e_j)}$ are permutation equivalent.
%\end{conj}
